Improving Scientific Hypothesis Generation with Knowledge Grounded Large Language Models

Large language models (LLMs) have demonstrated remarkable capabilities in various scientific domains, from natural language processing to complex problem-solving tasks. Their ability to understand and generate human-like text has opened up new possibilities for advancing scientific research, enabling tasks such as data analysis, literature review, and even experimental design. One of the most promising applications of LLMs in this context is hypothesis generation, where they can identify novel research directions by analyzing existing knowledge. However, despite their potential, LLMs are prone to generating ``hallucinations'', outputs that are plausible-sounding but factually incorrect. Such a problem presents significant challenges in scientific fields that demand rigorous accuracy and verifiability, potentially leading to erroneous or misleading conclusions. To overcome these challenges, we propose KG-CoI (Knowledge Grounded Chain of Ideas), a novel system that enhances LLM hypothesis generation by integrating external, structured knowledge from knowledge graphs (KGs). KG-CoI guides LLMs through a structured reasoning process, organizing their output as a chain of ideas (CoI), and includes a KG-supported module for the detection of hallucinations. With experiments on our newly constructed hypothesis generation dataset, we demonstrate that KG-CoI not only improves the accuracy of LLM-generated hypotheses but also reduces the hallucination in their reasoning chains, highlighting its effectiveness in advancing real-world scientific research.

==> contents/checklist.tex <==
\clearpage
\section{Reproducibility Checklist}

This paper:

\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes)
    \item Clearly delineates statements that are opinions, hypotheses, and speculation from objective facts and results (yes)
    \item Provides well-marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper (yes)
\end{itemize}

\noindent Does this paper make theoretical contributions? (no)

\noindent If yes, please complete the list below.

\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
    \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
    \item Proofs of all novel claims are included. (yes/partial/no)
    \item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
    \item Appropriate citations to theoretical tools used are given. (yes/partial/no)
    \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
    \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
\end{itemize}

\noindent Does this paper rely on one or more datasets? (yes)

\noindent If yes, please complete the list below.

\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets (yes)
    \item All novel datasets introduced in this paper are included in a data appendix. (yes)
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes)
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisfactory. (NA)
\end{itemize}

\noindent Does this paper include computational experiments? (yes)

\noindent If yes, please complete the list below.

\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. (yes)
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes)
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)
    \item All source code implementing new methods has comments detailing the implementation, with references to the paper where each step comes from. (yes)
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes)
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes)
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes)
    \item This paper states the number of algorithm runs used to compute each reported result. (yes)
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (no)
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (no)
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes)
    \item This paper states the number and range of values tried per (hyper-)parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (NA)
\end{itemize}


==> tables/case_study_llama_8B.tex <==
\begin{table*}[h]
    \centering
    \begin{tabular}{p{16.5cm}}
    \toprule
    \bf \makecell[c]{Hypothesis generation question} \\
    \midrule
    \textbf{Input}: Can we hypothesize a key relation between Acetylcysteine and MAPK1? \\
    \textbf{Ground Truth}: inhibit \\
    \midrule
    \rowcolor[RGB]{234, 238, 234}
    \bf \makecell[c]{Direct} \\
    \midrule
    \textbf{Answer}: no relation \textcolor{red}{\xmark} \\
    \midrule
    \rowcolor[RGB]{234, 238, 234}
    \bf \makecell[c]{CoT} \\
    \midrule
    \textbf{Reasoning}: Acetylcysteine is a precursor to glutathione, which is involved in the regulation of various cellular processes, including the MAPK signaling pathway. MAPK1 is a key component of this pathway. \hl{Additionally, research has shown that glutathione can modulate the activity of MAPK1.} \\
    \textbf{Answer}: stimulate \textcolor{red}{\xmark} \\
    \midrule
    \rowcolor[RGB]{234, 238, 234}
    \bf \makecell[c]{RAG} \\
    \midrule
    \textbf{Retrieved documents}: [...] \\
    \textbf{Reasoning}: Acetylcysteine is an antioxidant that can modulate various cellular processes, including those involving MAPK1. \hl{Research has shown that Acetylcysteine can influence the activity of MAPK1 in different contexts, such as in the regulation of cell growth and survival.} \\
    \textbf{Answer}: no relation \textcolor{red}{\xmark} \\
    \midrule
    \rowcolor[RGB]{234, 238, 234}
    \bf \makecell[c]{KG-CoI (Ours)} \\
    \midrule
    \textbf{Neighbor relations}:     (MAPK1, associate, Reactive Oxygen Species), (Reactive Oxygen Species, negative correlate, Acetylcysteine) \\
    \textbf{Retrieved documents}: [...] \\
    \textbf{Reasoning}: \hl{Acetylcysteine is an antioxidant that can neutralize reactive oxygen species, which are involved in the activation of MAPK1.} Therefore, it is likely that Acetylcysteine inhibits the activation of MAPK1. \\
    \textbf{Answer}: inhibit \greencheck \\
    \bottomrule
    \end{tabular}
    \caption{An example of how KG-CoI helps GPT-4o generate correct hypotheses and reduce hallucinations. We highlight reasoning steps that can be verified by KG. \guangzhi{this may not be a good example as there is no hallucination}}
    \label{tab:case_study}
\end{table*}

==> tables/property.tex <==
\begin{table*}
    \centering
    \begin{tabular}{cccccccc}
    \toprule
    Method & Llama-3.1-8B & Llama-3.1-70B & GPT-4o-mini & GPT-4o \\
    \midrule
    direct & -- & -- & -- & -- \\
    direct + SC & -- & -- & -- & -- \\
    CoT & 50.96 &  & 38.07 &  \\
    CoT + SC & 48.66 &  & 47.43 &  \\
    CoT + Iter & 45.59 & & 36.26 & \\
    KG-CoI & 66.84 &  & 42.70 &  \\
    KG-CoI + SC & 69.24 &  & 54.81 &  \\
    KG-CoI + Iter & 64.44 &  & 48.94 &  \\
    \bottomrule
    \end{tabular}
    \caption{Analysis of hallucination in hypotheses generated by different methods. \guangzhi{this table needs to re-designed to reflect hallucinations}}
    \label{tab:property}
\end{table*}

==> tables/scores.tex <==
\begin{table*}
    \centering
    \begin{tabular}{cccccccccccc}
    \toprule
        \multirow{3}{*}{\bf Method} & \multirow{3}{*}{\bf Knowledge} & \multicolumn{2}{c}{\bf Llama-3.1-8B} & \multicolumn{2}{c}{\bf Llama-3.1-70B} & \multicolumn{2}{c}{\bf GPT-4o-mini} & \multicolumn{2}{c}{\bf GPT-4o} \\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
    & & Accuracy & F1 & Accuracy & F1 & Accuracy & F1 & Accuracy & F1 \\
    \midrule
    direct & No & 47.00 & 48.71 & 72.00 & 71.94 & 52.66 & 51.12 & 69.00 & 68.33 \\
    direct + SC & No & 55.33 & 53.92 & 51.85* &  & 70.67 & 70.37 & 68.67 & 68.14 \\
    CoT & No & 56.67 & 56.61 & 73.67 & 73.77 & 65.33 & 63.27 & 71.33 & 71.33 \\
    CoT + SC & No & 51.67 & 51.48 & 71.43* &  & 67.00 & 65.90 & 73.67 & 73.78 \\
    CoT + Iter & No & 56.67 & 57.22 & 78.31* &  & 75.00 & 74.79 & 83.33 & 83.71 \\
    KG-CoI & Yes & 70.33 & 70.42 & 79.33 & 79.52 & 79.33 & 78.72 & 85.00 & 84.60 \\
    KG-CoI + SC & Yes & 50.33 & 50.539 & 52.91* &  & 78.00 & 77.45 & 85.00 & 85.34 \\
    KG-CoI + Iter & Yes & 48.67 & 49.55 & 59.79* &  & 79.33 & 79.17 & 84.00 & 83.65 \\
    \bottomrule
    \end{tabular}
    \caption{Comparison of our proposed Knowledge Grounded Chain of Ideas (KG-CoI) and baseline methods on zero-shot hypothesis generation for biological knowledge. ``Knowledge'' denotes if the method is augmented with external biological knowledge. \guangzhi{merge table 2 to this table if we don't have too many methods to compare: each row becomes LLM-method, columns contain knowledge, ACC, f1, confidence}\guangzhi{finish this part first, and we can compare it with RAG* (RAG* means the direct evidence should be removed from the context.) The comparison of RAG can also be put in the appendix}}
    \label{tab:scores}
\end{table*}
